Lasagna: Layered Score Distillation for Disentangled Object Relighting

Professional artists, photographers, and other visual content creators use object relighting to establish their photo's desired effect. Unfortunately, manual tools that allow relighting have a steep learning curve and are difficult to master. Although generative editing methods now enable some forms of image editing, relighting is still beyond today's capabilities; existing methods struggle to keep other aspects of the image -- colors, shapes, and textures -- consistent after the edit. We propose Lasagna, a method that enables intuitive text-guided relighting control. Lasagna learns a lighting prior by using score distillation sampling to distill the prior of a diffusion model, which has been finetuned on synthetic relighting data. To train Lasagna, we curate a new synthetic dataset ReLiT, which contains 3D object assets re-lit from multiple light source locations. Despite training on synthetic images, quantitative results show that Lasagna relights real-world images while preserving other aspects of the input image, outperforming state-of-the-art text-guided image editing methods. Lasagna enables realistic and controlled results on natural images and digital art pieces and is preferred by humans over other methods in over 91% of cases. Finally, we demonstrate the versatility of our learning objective by extending it to allow colorization, another form of image editing.

==> sec/old/1_introduction_v1.tex <==
\section{Introduction}

State-of-the-art generative models have attained remarkable realism and expressive power and have the potential to become an indispensable tool for artists of various skill levels. 
% The majority of digital artists use specialized image editing applications, such as Adobe Photoshop~\cite{photoshop} and Procreate~\cite{procreate}, that allow a layered representation of images as illustrated in Figure~\ref{fig:layered_repr} in the Appendix.  
% Most artists prefer such layered representation since it disentangles different aspects of an image, \textit{e.g.}, outlines, colorized foreground and background, shading, lighting, textures, \textit{etc.}, which allows more flexible and fine-grained editing. 
Although recent works on text-guided image editing with diffusion models~\cite{mokady2023null,brooks2023instructpix2pix,kawar2023imagic} and generative transformers~\cite{chang2023muse} show impressive editing capabilities, language guidance has limited control of certain fine-grained features, such as lighting and shading, due to the lack of grounding prior in the language space. While specialized methods for these subtle geometry-aware edits exist~\cite{yeh2022learning, liao2015approximate, zhang2022simbar}, unlike the large-scale diffusion models for image generation, they are typically trained on the relatively small curated datasets for intrinsic estimation and therefore struggle to generalize to a wide range of domains. Introducing such fine-grained geometric prior via finetuning the diffusion model on synthetic data is one promising direction~\cite{michel2023object} for extending the editing capabilities of text-conditional models. However, as we show in this paper, direct application of a finetuned model is not suitable for fine-grained edits, such as relighting, that require all aspects of the input image not related to lighting to be fixed. In this paper, we propose an image editing method, \MethodName, that leverages the relighting prior of a finetuned diffusion model to perform accurate and controlled single-view object relighting and surpasses the need to accurately estimate the geometric properties of an object, performing the disentangled relighting in the 2D space. 
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{sec/img/teaser.pdf}
    \caption{Given a single input image (\textit{top row}) and a text prompt specifying a lighting condition (e.g. light pointing from the left and right sides in the \textit{second and third rows}, respectively), \MethodName~ performs geometry-aware relighting of images of various levels of realism, from natural photos to minimalist digital art, and allows text-guided light conditioning.}
    \label{fig:teaser}
\end{figure}
\MethodName~ achieves disentangled shading by leveraging the prior of a fine-tuned diffusion model and a layer composition function that restrict the edit to a certain functionality. For example, shading layer, or ``multiply" layer commonly used in image editing tools like Photoshop~\cite{photoshop} and Procreate~\cite{procreate}, is composed via adjusting the luminosity of the input image -- multiplying the luminosity of the base layer with the shading layer. Such functional composition restricts the edit to only adjust the luminosity of the input image without changing other aspects of the image, such as color intensity or the overall layout. Inspired by DreamFusion~\cite{poole2022dreamfusion} that learned a text-to-3D generation using the diffusion model prior, in \MethodName, we extract the relighting prior of a finetuned model via the score distillation sampling. 

Our contributions can be summarized as follows:
\begin{itemize}
    \item We propose a disentangled image editing method, \MethodName, for layered image editing. \MethodName~ leverages generative prior of a diffusion model via score distillation sampling and disentangles the edit via a layer composition function. To the best of our knowledge, \MethodName~ is the first image editing method that successfully uses score distillation sampling.
     \item We introduce a novel Objaverse-R dataset for relighting based on the popular Objaverse dataset~\cite{deitke2023objaverse} of a variety of 3D objects. The proposed synthetic Objaverse-R dataset helps a diffusion model learn a robust association between the language guidance and the lighting conditions.
    \item We illustrate the advantages of using \MethodName~ on the relighting task compared to the popular text-guided image editing methods. Since the language control for lighting and shading are limited in popular diffusion models, we introduce the language-guided relighting prior by finetuning a ControlNet~\cite{zhang2023adding} adapter on Objaverse-R. We show that finetuning on synthetic data introduces a language-based relighting prior that generalizes to a wide range of image domains, including natural images and digital art of various levels of abstraction.
\end{itemize}
% In this paper, we propose \MethodName, a \emph{layered image editing} method that achieves disentangled sampling and editing by restricting the edit via a layer composition function, which 

\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{sec/img/controlled_relighting.png}
    \caption{With \MethodName, we can perform controlled relighting with language guidance only. Given a simple language prompt that specifies the lighting direction, ~\MethodName~ performs shape-aware relighting and generalizes to both natural images and digital art examples of various levels of abstraction.}
    \label{fig:controlled_res}
\end{figure*}


==> sec/old/1_introduction_v2.tex <==
\section{Introduction}

%\ar{I think the intro should follow this narrative:
%- image to image editing with text is a powerful capability - art, creativity, simulation. 
%- Current approaches achieve impressive text-based semantic editing but fail to perform controlled edits that %are not richly represented in training data - eg shading and relighting. 
%- Where are applications where relighting and shading required?
%    - photography - inserting an object into another image and making it fit. 
%    - 
%- Making controlled changes still requires the knowledge of how to use specialized tools like photoshop. 
%- We propose Lasagna - ....
%}

Image editing has become an indispensable skill in today's visual-centric world of social media and digital art. 
While professional image-editing tools such as Photoshop \cite{photoshop} and Procreate \cite{procreate} can make impressive edits, their steep learning curve is often daunting to novices in the field.
Amateur photographers and digital artists today desire intuitive tools to turn their art-in-progress into visual masterpieces.

Recently, generative image models \cite{brooks2023instructpix2pix, kawar2023imagic, hertz2022prompt} have been heralded as a promise to abstract out the minutiae of tedious pixel-level edits and provide an intuitive natural-language interface.
While these models have impressive capabilities to generate novel compositions \cite{}, they fail to make controlled physics-aware edits like shading and relighting to custom objects. 
In contrast to generating new images, controlled edits give artists more expressive freedom. For instance, they can insert a new object of their creation in a scene and tell the AI in natural language to match the lighting and shading of the object to the scene.

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{sec/img/teaser.pdf}
    \caption{\MethodName~ relights a input image with a precise control over light source position using a \emph{text guidance} only and performs shape-aware relighting of images of various levels of realism, from natural photos to minimalist digital art.}
    \label{fig:teaser}
\end{figure}

Recent works on natural language-guided image editing can accurately edit colors, textures, and attributes of objects \cite{brooks2023instructpix2pix, hertz2022prompt, bar2022text2live}. 
However, these models are usually trained with alt-text descriptions of images found on the web, and the text commonly describes the image's content rather than physics-aware parameters of the photo such as light direction and intensity.
Hence, along with contemporary work \cite{michel2023object}, we observe that existing image generation models fail to make controlled edits on physics-aware features such as lighting and shading. 

Hence, to enable fine-grained physics-aware edits such as relighting and shading, we propose \MethodName{}, a layered editing approach that learns to edit a disentangled shading or relighting layer on real images without using any real data. 
We learn how the light direction affects the lighting and shading of an object in simulation and distill the knowledge to apply it to real images. 
Compared to recent approaches that require reasoning about the object in the 3D space \cite{liao2015approximate}, we distill from 3D simulators to directly operate in the 2D image regime during test-time editing, reducing the complexity of the pipeline. 
The closest approach to ours uses 3D simulators to learn edits for moving objects in the scene \cite{michel2023object}. In contrast, we focus on learning the edits for moving the light direction in a scene. Moving the light direction may be simpler than moving objects, however, we see that models still fail to accurately edit the effect of lighting. 
Moreover, we believe that giving artists an additional control knob for lighting is rooted in practical applications where they may want to change the shading of an object they drew rather than move it around.


\MethodName{} achieves realistic physics-aware edits by distilling the knowledge from 3D simulations. 
Generative models trained directly on 3D simulations are likely to overfit since simulated images have a starkly different distribution to real images.
Hence, we first learn a shading model by fine-tuning on lighting-direction-based edits in a simulation. 
Next, we use the shading model's prior and learn to generate a shading layer for a light direction on real images. 
A crucial component of our approach is editing just a shading layer which restricts the edit to a certain functionality.
This allows us to perform realistic edits using a shading model trained without any real images and prevents changing other aspects of the image, such as color intensity or the overall layout. 

\MethodName{} is powered by \DataName{} - a large-scale data of $N$(todo: fill in) images of $X$(todo: fill in) 3D objects \underline{reli}ghted and \underline{sh}aded with 12 different directions along with the original object with diffused lighting (no shading).
We compute the mean-squared error of our edits on a held-out test set of \DataName{} and show that we perform better than existing text-guided image editing approaches. 

In sum, our contributions are as follows:



==> sec/old/1_introduction_ver_ar.tex <==
\section{Introduction}
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{sec/img/teaser_with_baselines.pdf}
    \caption{\small{Given a single input image (\textit{top row}) and a text prompt specifying a lighting condition (e.g. light pointing from the left and right sides in the \textit{bottom rows}, respectively), \MethodName~ performs geometry-aware relighting of images of various levels of realism, from natural photos to minimalist digital art, and allows text-guided light conditioning. State-of-the-art InstructPix2Pix~\cite{brooks2023instructpix2pix} (\textit{second row}), given the prompt that works best in our experiments, struggles to perform realistic relighting, while ControlNet~\cite{zhang2023adding} (\textit{third row}) trained on relighting data often alters crucial aspects of the image. \ranjay{The light direction is too small and unintuitive in this diagram. Also I recommend have the rows be (1) input, (2) lasagna, (3) lasagna, white space, (4) InstructPix2Pix, (5) controlnet.}}}
    \label{fig:teaser}
\end{figure}




Image editing requires a wealth of knowledge about the 3D scene - the geometry of objects, their position, and how the direction and type of lighting affect their appearance. 
Manual editing tools like Photoshop \cite{photoshop} and Procreate~\cite{procreate} can perform such edits; however, the process is often tedious and time-consuming to novices and professionals alike. While specialized methods for relighting and shading exist~\cite{yeh2022learning, liao2015approximate, zhang2022simbar}, they rely on complicated pipelines to estimate object intrinsics and lack an intuitive natural language interface.
Recent diffusion model-based editing methods ~\cite{mokady2023null,brooks2023instructpix2pix,kawar2023imagic} promise to offer a more straightforward and human-friendly language-based conditioning, but they have limited control of the geometry-aware features, such as lighting, shading or reflection, due to a lack of such knowledge in their language pre-training.
As shown in Figure \ref{fig:teaser}, if we instruct a state-of-the-art image editing method InstructPix2Pix\cite{brooks2023instructpix2pix} to relight given objects, it fails to control light direction, apply realistic relighting in general, as well as to preserve the overall appearance and content of the input image. 
One effective way to improve specific editing capabilities is finetuning with supervision, however, real datasets for relighting are typically too small to allow generalization ~\cite{murmann2019dataset,toschi2023relight}. 
Finetuning on synthetic data has shown to be a promising alternative~\cite{michel2023object} for geometry-aware edits. However, as shown in Figure~\ref{fig:teaser}, directly applying a model trained on synthetic data for relighting on the out-of-distribution examples often leads to undesired changes other crucial aspects of the input, such as colors, textures and background.
% In contrast, our layered-edit mechanism only allows the model to change the relevant aspects, also making it easier for the sythetic-data tuned model to only edit the required changes rather than re-rendering the entire scene. 

Hence, to provide artists with an intuitive language-based tool to perform subtle and geometry-aware edits such as relighting, we propose \MethodName, an approach for disentangled and restricted image editing. Inspired by DreamFusion~\cite{poole2022dreamfusion} that learns a text-to-3D generation using a diffusion model prior, in \MethodName, we extract the relighting prior of the diffusion model via score distillation sampling. \MethodName{} leverages the prior of a model tuned \textit{only} on synthetic images to perform controlled and geometrically accurate relighting with control of the lighting angle, achieving disentangled edits on images of various domains, as shown in Figure~\ref{fig:controlled_res}. Unlike methods that require estimating object geometry, \MethodName{} surpasses the need to accurately predict the object intrinsics, performing relighting directly in the pixel space. Moreover, unlike general text-guided image editing methods, \MethodName{} guarantees preservation of the input image content by restricting the editing layer to affect only the image luminosity. 

% For example, the shading layer, or ``multiply" layer commonly used in image editing tools like Photoshop~\cite{photoshop} and Procreate~\cite{procreate}, is composed via adjusting the luminosity of the input image -- multiplying the luminosity of the base layer with the shading layer. 
% Such functional composition restricts the edit to only adjust the luminosity of the input image without changing other aspects of the image, such as color intensity or the overall layout.
To train \MethodName{}, we propose \textbf{Objaverse-R}, a large-scale synthetic dataset built based on the popular Objaverse dataset \cite{deitke2023objaverse} and tailored for object relighting with control over light source location and direction. \textbf{Objaverse-R} helps a diffusion model to learn a robust association between the language guidance and the lighting direction and to disentangle it from other factors of variation. We show the efficacy of \MethodName{} on datasets from three different domains - natural photos from the Dreambooth dataset, digital art pieces, and the test set of the proposed Objaverse-R dataset. Our experimental results indicate a clear advantage of \MethodName~ over state-of-the-art text-guided image editing methods as well as the baseline finetuned for relighting, with our method being preferred in {\color{red} X percent of cases} according to the human evaluation study.

% Our contributions can be summarized as follows:
% \begin{itemize}
%     \item{We propose \MethodName~ for disentangled layered image editing. \MethodName~ leverages generative prior of a diffusion model via score distillation sampling and disentangles the edit via a layer composition function. To the best of our knowledge, \MethodName~ is the first image editing method that successfully uses score distillation sampling.}
%     \item{We introduce a novel synthetic \textbf{Objaverse-R} dataset for relighting containing 14K objects relighted in 12 different directions.}
%     \item{We show that, compared to the popular text-guided image editing methods, \MethodName~ performs controlled relighting while preserving other aspects of the input image and generalizes to a wide range of image domains, including natural images and digital art of various levels of abstraction.}
% \end{itemize}
% In this paper, we propose \MethodName, a \emph{layered image editing} method that achieves disentangled sampling and editing by restricting the edit via a layer composition function, which 

\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{sec/img/controlled_relighting.png}
    \caption{\small With \MethodName, we can perform controlled relighting with language guidance only (light direction shown at the top). Given a simple language prompt that specifies the lighting direction, ~\MethodName~ performs shape-aware relighting and generalizes to both natural images and digital art examples of various levels of abstraction. }
    \label{fig:controlled_res}
\end{figure*}


==> sec/old/1_introduction_ver_ar_2.tex <==
\section{Introduction}

Realistic image editing requires a wealth of knowledge about the 3D scene - the geometry of objects, their position, and how the direction and type of lighting affect their appearance. 
Manual editing tools like Photoshop \cite{photoshop} and Procreate~\cite{procreate} can perform such edits; however, the process is often tedious and time-consuming to novices and professionals alike. While specialized methods for relighting and shading exist~\cite{yeh2022learning, liao2015approximate, zhang2022simbar}, they rely on complicated pipelines to estimate object intrinsics and lack an intuitive natural language interface.

Recent diffusion model-based editing methods ~\cite{mokady2023null,brooks2023instructpix2pix,kawar2023imagic} promise to offer a more human-friendly language-based interface, but we observe that they underperform on edits that require knowledge of the object's 3D geometry- such as the light direction and how that affects the shadows and reflections.
As shown in Figure \ref{fig:teaser} (row 2), if we instruct a state-of-the-art image editing method InstructPix2Pix\cite{brooks2023instructpix2pix} to relight objects with ``lighting from the left'', it fails to accurately edit the shading and lighting, while preserving the appearance of the object. For example, the dog (col 1) is lit from the right, and the sesame on the burger disappears (col 4).  
We believe this might be due to a lack of geometry-aware editing knowledge in the language pre-training data of diffusion models.
Hence, finetuning on synthetic data for geometry-aware edits has shown to be a promising direction~\cite{michel2023object}. However, as shown in Figure \ref{fig:teaser} (row 3), directly applying a model trained on synthetic data for subtle image edits like relighting on real data often leads to undesired changes.
% In contrast, our layered-edit mechanism only allows the model to change the relevant aspects, also making it easier for the sythetic-data tuned model to only edit the required changes rather than re-rendering the entire scene. 
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{sec/img/teaser_with_baselines.pdf}
    \caption{\small{Given a single input image (\textit{top row}) and a text prompt specifying a lighting condition (e.g. light pointing from the left and right sides in the \textit{third and fourth rows}, respectively), \MethodName~ performs geometry-aware relighting of images of various levels of realism, from natural photos to minimalist digital art, and allows text-guided light conditioning. State-of-the-art Pix2Pix (\textit{second row}) struggles to perform the realistic relighting and often alters crucial aspects of the image, such as colors, textures and details.}}
    \label{fig:teaser}
\end{figure}

Hence, to provide artists with an intuitive language-based tool to perform subtle geometry-aware edits such as relighting, we propose \MethodName. \MethodName{} leverages the relighting prior of a diffusion model tuned \textit{only} on synthetic images to perform controlled and geometrically accurate relighting edits on real and generated images alike. Unlike the relighting methods that estimate the object intrinsics, \MethodName{} surpasses the need to accurately estimate the geometric properties of an object, performing relighting in the pixel space. Moreover, unlike general text-guided image editing methods, \MethodName{} guarantees the preservation of the content and appearance of the input image by restricting the editing layer to affect only the image luminosity. Inspired by DreamFusion~\cite{poole2022dreamfusion} that learns a text-to-3D generation using a diffusion model prior, in \MethodName, we extract the relighting prior of the diffusion model fine-tuned for relighting via score distillation sampling.  

% For example, the shading layer, or ``multiply" layer commonly used in image editing tools like Photoshop~\cite{photoshop} and Procreate~\cite{procreate}, is composed via adjusting the luminosity of the input image -- multiplying the luminosity of the base layer with the shading layer. 
% Such functional composition restricts the edit to only adjust the luminosity of the input image without changing other aspects of the image, such as color intensity or the overall layout.
To train \MethodName{}, we propose \textbf{Objaverse-R}, a large-scale procedurally generated dataset tailored to object relighting and shading. Our \textbf{Objaverse-R} is built on top of Objaverse \cite{deitke2023objaverse} and contains 169K object-images relight in 12 directions. We use \textbf{Objaverse-R} to fine-tune a diffusion model to learn an association between the language guidance and the lighting direction, which we further distill similar to Dreamfusion \cite{poole2022dreamfusion} to apply to real images as well.

Finally, we show the efficacy of \MethodName{} on datasets from three different domains - natural photos from the Dreambooth dataset, digital art pieces, and the test set of the proposed Objaverse-R dataset. We show that humans prefer \MethodName{} edits over state-of-the-art editing methods by $x\%$. 

Our contributions can be summarized as follows:
\begin{itemize}
    \item We propose \MethodName~ for disentangled layered image editing. \MethodName~ leverages the generative prior of a diffusion model via score distillation sampling and disentangles the edit via a layer composition function. To the best of our knowledge, \MethodName~ is the first image editing method that successfully uses score distillation sampling.
     \item We introduce a novel synthetic \textbf{Objaverse-R} dataset for relighting containing 14K objects relighted in 12 different directions. 
    \item We show that, compared to the popular text-guided image editing methods, \MethodName~ performs controlled relighting while preserving other aspects of the input image and generalizes to a wide range of image domains, including natural images and digital art of various levels of abstraction.
\end{itemize}
% In this paper, we propose \MethodName, a \emph{layered image editing} method that achieves disentangled sampling and editing by restricting the edit via a layer composition function, which 

\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{sec/img/controlled_relighting.png}
    \caption{\small With \MethodName, we can perform controlled relighting with language guidance only (light direction shown at the top). Given a simple language prompt that specifies the lighting direction, ~\MethodName~ performs shape-aware relighting and generalizes to both natural images and digital art examples of various levels of abstraction.}
    \label{fig:controlled_res}
\end{figure*}

